Privately Learning High-Dimensional Distributions

We present novel, computationally efficient, and differentially private algorithms for two fundamental high-dimensional learning problems: learning a multivariate Gaussian and learning a product distribution over the Boolean hypercube in total variation distance. The sample complexity of our algorithms nearly matches the sample complexity of the optimal non-private learners for these tasks in a wide range of parameters, showing that privacy comes essentially for free for these problems. In particular, in contrast to previous approaches, our algorithm for learning Gaussians does not require strong a priori bounds on the range of the parameters. Our algorithms introduce a novel technical approach to reducing the sensitivity of the estimation procedure that we call recursive private preconditioning.

==> univariate.tex <==
\section{Tighter Bounds for Univariate Gaussian Mean Estimation}

In this section we give an algorithm for univariate Gaussian mean estimation that slightly improves over the algorithm from~\cite{KarwaV18} by removing certain polylogarithmic factors.  Suppose we are given i.i.d.\ samples $X_1,\dots,X_n \sim \normal(\mu,1)$ with the promise $|\mu| \leq R$.  Our algorithm uses two main steps, the first of which is identical to~\cite{KarwaV18}, but the second of which is different.
\begin{enumerate}
\item Privately find a weak estimate $\wt\mu$ such that $| \mu - \wt\mu | = O(1)$.  As in~\cite{KarwaV18}, we do this (roughly) by rounding samples to the nearest integer in $[-R,R]$ and then privately computing a histogram of the rounded samples.  We then set $\wt\mu$ to be the most frequent value in the private histogram, which satisfies the accuracy requirement with high probability.

\item Privately compute $\wt p \approx \frac1n \sum_{i=1}^{n} \mathbf{1}\{ X_i \leq \wt\mu \}$.  Note that this quantity converges to $$p = \pr{}{\normal(\mu,1) \leq \wt\mu} = \Phi(\wt\mu - \mu)$$ where $\Phi$ is the CDF of the standard normal distribution.  Then output $\wh\mu = \wt\mu - \Phi^{-1}(\wt p)$.  As a sanity check, note that $\mu = \wt\mu - \Phi^{-1}(p)$, so as $\wt p \to p$ we have $\wh\mu \to \mu$.
\end{enumerate}

First we recall the following differentially private algorithm for computing histograms, which is one of the key tools in our algorithm.
\begin{theorem}[\cite{BeimelNS13,Vadhan17,BunS16}]
\label{thm:private-histogram}
For every universe $\cX$, $n \in \N$, $0 < \eps$ and $\delta,\beta \in (0,\frac1n)$,
there is a polynomial time $(\eps, \delta)$-DP mechanism $H_{\eps,\delta} : \cX^n \to \R^\cX$ such that, for every $X \in \cX^n$, with probability at least $1 - O(\beta)$,
$$
\left\| q(X) - H_{\eps,\delta}(X) \right\|_{\infty} \leq O\left( \frac{\log(\frac{1}{\delta\beta})}{\eps n} \right)
$$
where
$q_{y}(X) = \frac1n \sum_{i = 1}^{n} \mathbf{1}_{y}(X_i)$.
Moreover, for every $\rho > 0$ there is an analogous $\rho$-zCDP algorithm $H_{\rho}$ such that with probability at least $1 - O(\beta)$,
$$
\left\| q(X) - H_{\rho}(X) \right\|_{\infty} \leq O\left( \frac{\sqrt{\log\left(\frac{|\cX|}{\beta}\right)}}{\rho^{1/2} n} \right)
$$
\end{theorem}

To define our algorithm, let $I_{r} = (r,r+1)$ and define the domain 
$$\cX_{R} = \set{ I_{r} : r = -R,\dots,R-1 }$$
Given a sample $X_i$, we define
\begin{equation*}
B_i = 
\begin{cases}
I_r & \textrm{if $X_i \in I_{r}$ for some $r = 1,\dots,2R$}\\
I_{-R} & \textrm{if $X_i < -R$} \\
I_{R-1} & \textrm{if $X_i > R$}
\end{cases}
\end{equation*}
and given a dataset $X_1,\dots,X_n$ we define $B = (B_1,\dots,B_n)$.

\begin{algorithm}[h!]
\caption{Private Mean Estimator $M_{\rho}(X_1,\dots,X_{n+m})$}
\KwIn{Samples $X_1,\dots,X_{n+m} \in \R$ from a Gaussian $\normal(\mu, 1)$ with unknown mean $\mu \in (-R,R)$.  Parameters $\rho,\alpha,\beta > 0$.}
\KwOut{An estimate $\wh\mu$ such that $|\mu - \wh\mu| \leq \alpha$.}
\vspace{10pt}
Let $B_1,\dots,B_n,\cX_{R},H_{\rho}$ be as above and let $h \gets H_{\rho}(B_1,\dots,B_n)$.\\
\eIf{there exists $I_{r}$ such that $h_{I_{r}} \geq 1/4$}{$\wt\mu \gets r$}{\Return $\bot$}\vspace{10pt}

Let $\wt p \gets \frac1n \sum_{i=n+1}^{n+m} \mathbf{1}\{X_i \leq \wt \mu\}$\\
Let $\wh p \gets \wt p + \normal(0, \frac{1}{2\rho n^2})$\\ \vspace{10pt}
\Return $\wh\mu = \wt\mu - \Phi^{-1}(\wh p)$
\end{algorithm}

